Dynamic Inference on Graphs using Structured Transition Models

Enabling robots to perform complex dynamic tasks such as picking up an object in one sweeping motion or pushing off a wall to quickly turn a corner is a challenging problem. The dynamic interactions implicit in these tasks are critical towards the successful execution of such tasks. Graph neural networks (GNNs) provide a principled way of learning the dynamics of interactive systems but can suffer from scaling issues as the number of interactions increases. Furthermore, the problem of using learned GNN-based models for optimal control is insufficiently explored. In this work, we present a method for efficiently learning the dynamics of interacting systems by simultaneously learning a dynamic graph structure and a stable and locally linear forward model of the system. The dynamic graph structure encodes evolving contact modes along a trajectory by making probabilistic predictions over the edges of the graph. Additionally, we introduce a temporal dependence in the learned graph structure which allows us to incorporate contact measurement updates during execution thus enabling more accurate forward predictions. The learned stable and locally linear dynamics enable the use of optimal control algorithms such as iLQR for long-horizon planning and control for complex interactive tasks. Through experiments in simulation and in the real world, we evaluate the performance of our method by using the learned interaction dynamics for control and demonstrate generalization to more objects and interactions not seen during training. We introduce a control scheme that takes advantage of contact measurement updates and hence is robust to prediction inaccuracies during execution.

==> experiments.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/pickup_tasks_plots.pdf}
    \caption{(a) Row 1: Box2D Task 1 with same number of objects as seen during training. Row 2: Box2D Task 1 generalization scenario with many distractor objects (orange) in the scene. Row 3: Box2D Task 2 with same number of objects as seen during training. Row 4: Box2D Task 2 generalization scenario for picking up many more objects than during training. (b) 10-step root mean square error between the predicted and executed trajectories. These experiments are performed with the same number of objects and interactions as seen during training. (c) 10-step root mean square error between the predicted and executed trajectories. These experiments are performed to test for generalization by including many more objects and interactions in the task than seen during training. \todo{make row 2 last frame transparent. Motion of gripper and objects is depicted by overlayed transparent frames. }}
    \label{fig:box2d_and_error}
\end{figure*}
\section{EXPERIMENTS}
The proposed method is evaluated in simulation using Box2D and Isaac Gym environments and in the real-world on the 7DOF Franka-Emika Panda robot arm. Through our experiments, we aim to evaluate 1) How useful is our graph inference module in enabling efficient and accurate learning of the dynamics of the interactive system? 2) What are the generalization properties of the learned dynamics model as more objects (not seen during training) are added to the system? 3) How robust is our execution strategy to inaccuracies in the learned model?  4) Can our learned stable linearized dynamics be used for learning the cost function of a differentiable LQR controller using expert demonstrations of a task? \todo{hammer in the efficient learning stuff more - graph inference module reduces need for too much data}

\textbf{Ablation studies:} To answer the first three questions, we perform the following three ablation studies:
1) Training the dynamic model without the graph inference module i.e. learning the forward dynamics module given fully connected graphs. The dataset for this study is the same as the dataset used for training the full model. We call this model \textbf{No-GIM}. 2) Training the dynamic model without the graph inference module but with an augmented dataset containing more objects. We call this model \textbf{No-GIM-Aug}. 3) Training the full dynamic model with the graph inference module but replacing the GRU in \eqref{eq:gru} with a fully connected neural network that takes as input only the current edge embedding $\mathbf{m}_t^{ij}$ to output the edge activation i.e. there no temporal relationship between the predicted edge activations. We call this model \textbf{GIM-Non-Temp}. Due to this modification in the network architecture, we will no longer be able to utilize the robust control scheme elaborated in \ref{sec:exec}. We call our model \textbf{GIM-Temp}. To answer question 4, we learn the cost matrices $Q$ and $R$ of a discrete-time linear quadratic regulator (LQR) and demonstrate generalization of learned expert behavior to goal regions not visited by the expert.

\textbf{Evaluation metrics:} To test for generalization, all methods are tested with more objects and interactions than seen during training. For evaluating the accuracy of the learned model, the generalization properties and the effectiveness of the robust control scheme, we use 10-step prediction error as the metric. This error is calculated upon using the learned linearized models for control using iLQR-MPC and calculating the root mean square error between the predicted trajectory and the executed trajectory for a rollout length of 10. The prediction error is calculated over all the nodes in the graph. For Ablation 3, in addition to 10-step prediction error, we also evaluate the accuracy of the predicted edge activations for a rollout length of 10 and compare it with our method. We get the ground truth edge activations by observing contacts during execution. Contact information is not used during training. For Ablation 2, we also present results for the sample complexity, i.e how much more interaction data is needed in order to achieve similar level of performance as with our method. This will demonstrate the efficiency of our method as compared to models where the graph inference module is not used.

% We evaluate this using sample complexity as a metric for efficiency and 1-step prediction error as the metric for accuracy.

We perform three tasks using the Box2D simulation environment and one task using the Isaac Gym environment containing a simulated Franka-Emika Panda robot arm. Fig. \ref{fig:box2d_and_error}(b) shows the 10-step prediction error when the learned models are tested in environments with the same number of objects and interactions as seen during training. Fig. \ref{fig:box2d_and_error}(c) shows the 10-step prediction error for generalization scenarios i.e. testing with more interactions and more distractor objects in the scene. Fig. \ref{fig:doors_and_accuracy}(b) shows the 10-step edge activation prediction accuracy.
% To keep things simple, the Ablation studies are performed using the Box2D environment and the Isaac Gym environment is used to demonstrate our results on a highly non-linear system for tasks involving multiple dynamic modes and contacts.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/results.png}
%     \caption{10-step prediction error (MSE)}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/results_gen.png}
%     \caption{10-step prediction error - generalization (MSE)}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/results_mode.png}
%     \caption{Edge activation prediction accuracy (\%)}
%     \label{fig:my_label}
% \end{figure}
\subsubsection{Box2D Task 1: Dynamic pickup of one object with distractor objects}
We consider the task of dynamically (without stopping) picking up a 2D object using a 2D gripper and taking it to a goal region (Fig. \ref{fig:box2d_and_error}(a) Rows 1 \& 2). The simulation environment is setup such that when two objects come in contact they undergo a purely inelastic collision and a rigid link is formed between them, thus simulating grasping. First, we collect data such that, in each trajectory, the gripper picks up only one object, i.e. there are only two nodes in the training graphs; the gripper and one object node. Therefore, only one interaction occurs in this dataset. We sample the location of the gripper, object and the goal to collect the data. Using this data, we train dynamic models using our method and the methods described for Ablations 1 and 3. Then, we augment the data and add three distractor objects (that do not interact with the gripper or target object) to the trajectories and train using the method described for Ablation 2. All these learned models are then tested for generalization in environments containing upto \textit{ten} distractor objects, i.e. the states of the distractor objects are added as additional nodes in the graph. The aim here is to test generalization to distractor objects that do not interact. 

We use the learned interaction dynamics for control using iLQR-MPC and calculate the 10-step prediction error as shown in Fig. \ref{fig:box2d_and_error}(b \& c). We observe that the 10-step prediction error for all the models is comparable \todo{quantitative} when tested with only one object in the scene as shown in Fig. \ref{fig:box2d_and_error}(b). However, when tested for generalization, the performance of Ablation 1 deteriorates significantly as shown in Fig. \ref{fig:box2d_and_error}(c). This is because Ablation 1 never encounters distractor objects during training and with the absence of the graph inference module it cannot infer that the distactor objects do not interact and edges to them can be rendered inactive. In comparison, Ablation 3 and our model also do not encounter distractor objects during training but learn to ignore them by rendering the edges to them inactive. We also observe that Ablations 2 and 3 perform similarly well and even generalize well. The augmented data helps the model for Ablation 2 infer the role of distractor objects as non-interacting nodes, however, this comes at the cost of four times as much data and longer training time. \todo{add training curve to supplementary material and point to it?}

The 10-step prediction error of our model is lower than that of all other models. This demonstrates the benefit of using GRU and our robust execution strategy that adapts to observed contact events. Both Ablation 3 and our method were are able to infer that an active edge exists between the gripper node and the target object node only after contact has occurred. The edge activation prediction accuracy of our model is 100\% because of reactive update during execution as compared to 89\% for Ablation 3 \ref{fig:doors_and_accuracy}(b). Ablation 3 shows inaccuracies especially in regions close to contact. 

% This allows the controller plan more accurately for the changing dynamics and start applying more force for pickup right after contact is made. Thus, our control scheme yields a much smoother and robust execution of the task. 

Finally, we use our learned model to learn the quadratic cost matrices of a LQR controller using the method described in \ref{sec:cost}. We learn the cost function for \textit{dynamically} picking up a 2D object using a 2D gripper and taking it to a fixed goal region. Expert demonstrations are collected by sampling the initial position for the gripper and keeping the goal and object locations fixed. Our aim is to evaluate if the learned controller mimics the behavior of the expert and if it generalizes to unseen goal and object locations. We evaluate the performance of the learned controller using task success as the metric. If the gripper is able to pick up the object and take it within a goal region in time T then the task is considered successful. We observe that the learned controller can perform the task with \todo{98\%} success rate. \todo{add gif to supplementary material and point to it?}

\todo{Also add qualitative results info about the modes that are detected, plots can be added to supplementary material}

\subsubsection{Box2D Task 2: Dynamic pickup of multiple objects}
We consider the task of dynamically picking up two 2D objects using a 2D gripper and taking them to a goal region (Fig. \ref{fig:box2d_and_error}(a) Rows 3 \& 4). We collect interaction data such that the gripper picks up either one or both the objects and takes them to a goal region. Thus, the training graphs contain a maximum of three nodes (gripper and two objects) at any time step. Using this data, we train the dynamic model using our method and the method described for Ablations 1 and 3. Similar to task 1, we augment the data with two more object interactions to train Ablation 2. All these learned models are then tested on tasks involving picking up more than two and upto five objects. The aim here is to test generalization to more than two interactions, not seen during training. The 10-step prediction error for all these models are again shown in Fig. \ref{fig:box2d_and_error}(b \& c). We observe here that the 10-step prediction error of all the ablation models is comparable \todo{quantitative} with Ablation 3 performing slightly better, when tested with only two objects \ref{fig:box2d_and_error}(b). However, when tested for generalization, the performance of model predictions in Ablation 1 suffers \ref{fig:box2d_and_error}(c). For this task as well, Ablation 2 performs similar to Ablation 3 because the augmented data helps the model generalize to more objects, but at the cost of higher sample complexity (three times the data) and higher training time. Our model outperforms other models and generalizes well. Both Ablation 3 and our model predict that edges between gripper and distractor objects are inactive and edges between the gripper and target objects becomes active when the objects are picked up. We again observe that the 10-step edge activation prediction accuracy of our model is higher as compared to Ablation 3 (\ref{fig:doors_and_accuracy}(b)) owing to the reactive edge updates during execution.
\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/doors_and_mode.pdf}
    \caption{(a) Row 1: Box2D Task 3 with same number of doors as seen during training. Row 2: Box2D Task 3 generalization scenario with many distractor doors in the scene. (b) 10-step edge activation prediction accuracy. \todo{add "10 step" on plot}}
    \label{fig:doors_and_accuracy}
\end{figure*}
\subsubsection{Box2D Task 3: Dynamic door opening}
We consider the task of dynamically opening a 2D door to a goal angle using a 2D gripper (Fig. \ref{fig:doors_and_accuracy}(a)). For this task, we collect data such that each trajectory is composed of one gripper opening one door i.e. all the training graphs have only two interacting nodes. Using this data, we train Ablations 1 and 3 and our model. We choose not to train Ablation 2 for the rest of the experiments since training it is expensive and gives comparable performance to Ablation 3. The aim of this experiment is to evaluate the learned stable locally linear dynamics model of a non-linear system by using the learned dynamics for control. To test for generalization, all the learned models are tested in environments containing upto ten distractor doors. For this task as well, we observe that the 10-step prediction error for all the models is good \todo{quantitative} when tested with only one door in the scene as shown in Fig. \ref{fig:box2d_and_error}(b). However, when tested for generalization, the performance of Ablation 1 deteriorates significantly as shown in Fig. \ref{fig:box2d_and_error}(c) again due to the fact that Ablation 1 never encounters distractor objects during training. Our method performs better than both Abalation 1 and 3. We observe the 10-step edge activation prediction accuracy of our model is higher ($100\%$) as compared to Ablation 3 ($97\%$) as shown in Fig. \ref{fig:doors_and_accuracy}(b).

\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/franka_tasks.pdf}
    \caption{(a) Isaac Gym Task 1 with same number of objects as seen during training. (b) Isaac Gym Task 1 generalization scenario with many distractor (green) objects in the scene. (c) Real world experiments with the 7DOF Franka-Emika Panda arm performing a dynamic pickup task using our learned model.}
    \label{fig:franka_tasks}
\end{figure*}

\subsubsection{Isaac Gym Task 1: Dynamic pickup of heavy object using Franka arm}
\label{sec:isaac1}
We consider the task of dynamically picking up a heavy object using a 7DOF Franka-Emika Panda arm in simulation (Fig. \ref{fig:franka_tasks}(a) and (b)). This task was designed such that the gripper slows down but does not completely stop before picking up the object. The object is made intentionally heavy so that there is a considerable change in the robot dynamics upon pickup and higher forces are needed to maintain the same z-location. We control the robot using task space impedance control during data collection and the orientation of the gripper is kept fixed. We collect data by sampling the cartesian space initial position of the object (on a table) and also the goal location. We save the cartesian space position and velocity of the gripper and the object, and also the cartesian force applied in the task frame. Using this data, we train dynamic models using our method and the methods described for Ablations 1 and 3. We use the learned interaction dynamics for control using iLQR-MPC and observe 10-step prediction error for the pickup task. We also add distractor objects to the scene and add them as nodes in the graph to test for generalization. Due to lack of reliable contact sensing, we do not update edge activation predictions using observed contacts during execution but still rely solely on GRU for edge activation predictions. We observe good \todo{quantitative} performance of each of the trained models for the pickup task (Fig. \ref{fig:box2d_and_error}(b)). However, when distractor objects are added to the scene as shown in Fig. \ref{fig:franka_tasks}(b), the model trained for Ablation 1 performs very badly and is not even able to successfully pick up the object in many scenarios. Both Ablation 3 and our model generalize well in the presence of distractor objects.

\subsubsection{Isaac Gym Task 2: Dynamic pickup of heavy object with table interactions using Franka arm}

\subsubsection{Real robot experiments}
Real world experiments are performed for the task of dynamically picking up a heavy object and taking it to a goal location using a 7DOF Franka-Emika Panda robot arm (Fig. \ref{fig:franka_tasks}(c)). Here again, the object is heavy thus there is a considerable change in the robot dynamics upon pickup and higher forces are needed to maintain the same z-location. \todo{reword this to not make it look it modes wont be detected if object is now} The setup, controller and data collection strategy is the same as for the Isaac Gym Franka pickup task discussed in \ref{sec:isaac1}. The location of the object was tracked using April tags and a Kinect depth sensor \cite{wang2016apriltag}. Again, due to lack of reliable contact sensing, we do not update edge activation predictions using observed contacts during execution but still rely solely on GRU for edge activation predictions. Using the collected data, we train Ablation 1, 3 and our model. We observe that since we do not use contact information for updating the edge predictions in our method, the performance of our method compared to the Abalation studies is not as good as in the other tasks. However, using iLQR-MPC with our learned linear model, we were able to perform the pickup task successfully as shown in Fig. \ref{fig:franka_tasks}(c).
